Handling Scope Checks (Extended Version)

Metaprogramming and effect handlers interact in unexpected, and sometimes undesirable, ways. One example is scope extrusion: the generation of ill-scoped code. Scope extrusion can either be preemptively prevented, via static type systems, or retroactively detected, via dynamic checks. Static type systems exist in theory, but struggle with a range of implementation and usability problems in practice. In contrast, dynamic checks exist in practice (e.g. in MetaOCaml), but are understudied in theory. Designers of metalanguages are thus given little guidance regarding the design and implementation of checks. We present the first formal study of dynamic scope extrusion checks, introducing a calculus ($\lambda_{\langle\langle\text{op}\rangle\rangle}$) for describing and evaluating checks. Further, we introduce a novel dynamic check $\unicode{x2014}$ the "Cause-for-Concern" check $\unicode{x2014}$ which we prove correct, characterise without reference to its implementation, and argue combines the advantages of existing dynamic checks. Finally, we extend our framework with refined environment classifiers, which statically prevent scope extrusion, and compare their expressivity with the dynamic checks.

==> sty/scope-colours.tex <==
\definecolor{linkcolor}{HTML}{019EC9}

\definecolor{ocamlBackground}{HTML}{FFF8F2}
\definecolor{ocamlHighlight}{HTML}{E9712C}

\definecolor{effBackground}{HTML}{F7F3FF}
\definecolor{effHighlight}{HTML}{582E9B}
\definecolor{effComment}{HTML}{9C75EB}


\definecolor{sourceBackground}{HTML}{E8F6FF}
\definecolor{sourceHighlight}{HTML}{00489A}
\definecolor{sourceComment}{HTML}{507FB4}

\definecolor{sourceHighlight2}{HTML}{1C428A}
\definecolor{sourceHighlight3}{HTML}{34548F}
\definecolor{sourceHighlight4}{HTML}{456196}


\definecolor{coreBackground}{HTML}{EBFCEE}
\definecolor{coreHighlight}{HTML}{006E6E}
\definecolor{coreComment}{HTML}{46A58F}

\definecolor{recBackground}{HTML}{FFE7E8}
\definecolor{recHighlight}{HTML}{83002C}

\definecolor{envclassifier1}{HTML}{E3E4E7}
\definecolor{envclassifier2}{HTML}{EBEBEC}
\definecolor{envclassifier2a}{HTML}{049CAF}
\definecolor{envclassifier3}{HTML}{C03A2A}

\definecolor{theorembar}{HTML}{323239}
\definecolor{comment}{HTML}{9999A0}

\definecolor{compile}{HTML}{FFA126}
\definecolor{quote}{HTML}{E60932}
\definecolor{splice}{HTML}{00CC52}

\definecolor{fade}{HTML}{EAEAEC}
\definecolor{stdout}{HTML}{F0F0F2}


\definecolor{lightgrey}{HTML}{CBCBCC}
\definecolor{darkgrey}{HTML}{848486}

\definecolor{selected}{HTML}{0362D1}
\definecolor{selectedTarget}{HTML}{3484E2}

\definecolor{fadedYellow}{HTML}{FFF4BA}

\definecolor{quotation}{HTML}{9999A0}

==> sty/scope-macros.tex <==
\definecolor{listing-quote}{HTML}{DC5B25}
\definecolor{listing-keyword}{HTML}{009128}
\definecolor{listing-constructor}{HTML}{002FFF}

\makeatletter
\newcommand*\listingfontsize{%
  \@setfontsize\listingfontsize{7}{8}%
}
\makeatother

\lstdefinestyle{style}{%
  % backgroundcolor=\color{white},
  basicstyle=\small\ttfamily,
  keywordstyle=\bfseries\color{listing-keyword},
  keywordstyle={[2]\bfseries\color{listing-constructor}},
  captionpos=none,
  columns=flexible,
  % baselinestretch=1.1,
  escapeinside=``,
  keepspaces=true,
  showspaces=false,               % show spaces adding particular underscores
  showstringspaces=false,         % underline spaces within strings
  showtabs=false,                 % show tabs within strings adding particular underscores
  breaklines=true,                % sets automatic line breaking
  breakatwhitespace=true,         % sets if automatic breaks should only happen at whitespace
  literate={lam}{{$\lambda$}}1  {->}{{$\rightarrow$}}1 {o+o}{{$\oplus$}}1 {=>}{{$\Rightarrow$}}1 {/\\}{{$\Lambda$}}1  {'a}{{$\alpha$}}1 {|}{{$\mid$}}1 {'\{}{'\{}1 {<-}{{$\leftarrow$}}1
    {<<}{{{\sffamily\color{listing-quote}<{}<}}}1
    {>>}{{{\sffamily\color{listing-quote}>{}>}}}1
    {\$}{{{\color{listing-quote}\$}}}1
  ,
  tabsize=2,
  commentstyle=\color{comment}\ttfamily,
  stringstyle=\color{red}\ttfamily,
  sensitive=true
}

\lstdefinestyle{lst_style}{%
  % backgroundcolor=\color{white},
  basicstyle=\listingfontsize\ttfamily,
  keywordstyle=\bfseries\color{listing-keyword},
  keywordstyle={[2]\bfseries\color{listing-constructor}},
  captionpos=none,
  sensitive=true,
  columns=flexible,
  % baselinestretch=1.1,
  numbers=left,
  numbersep=18pt,
  numberstyle=\scriptsize\ttfamily\color{comment},
  escapeinside=``,
  keepspaces=true,
  showspaces=false,               % show spaces adding particular underscores
  showstringspaces=false,         % underline spaces within strings
  showtabs=false,                 % show tabs within strings adding particular underscores
  breaklines=true,                % sets automatic line breaking
  breakatwhitespace=true,         % sets if automatic breaks should only happen at whitespace
  literate={lam}{{$\lambda$}}1  {->}{{$\rightarrow$}}1 {o+o}{{$\oplus$}}1 {=>}{{$\Rightarrow$}}1 {/\\}{{$\Lambda$}}1 {'a}{{$\alpha$}}1  {|}{{$\mid$}}1 {'\{}{'\{}1 {<-}{{$\leftarrow$}}1
    {<<}{{{\sffamily\color{listing-quote}<{}<}}}1
    {>>}{{{\sffamily\color{listing-quote}>{}>}}}1
    {\$}{{{\color{listing-quote}\$}}}1
  ,
  tabsize=2,
  commentstyle=\color{comment}\ttfamily,
  stringstyle=\color{red}\ttfamily,
}

\lstdefinestyle{plain}{%
  basicstyle=\listingfontsize\ttfamily,
  columns=flexible,
  escapeinside=``,
  keepspaces=true,
  showspaces=false,               % show spaces adding particular underscores
  showstringspaces=false,         % underline spaces within strings
  showtabs=false,                 % show tabs within strings adding particular underscores
  breaklines=true,                % sets automatic line breaking
  breakatwhitespace=true,         % sets if automatic breaks should only happen at whitespace
}

\lstdefinelanguage{plain}{xleftmargin  = 2mm}

\lstdefinelanguage{ocaml}{
  keywords={},
  morekeywords=[1]{and,as,asr,assert,begin,class,constraint,continue,do,done,downto,effect,else,end,exception,external,false,for,fun,function,functor,if,in,include,inherit,initializer,land,lazy,let,lor,lsl,lsr,lxor,macro,match,method,mod,module,open,perform,mutable,new,nonrec,object,of,open,open!,or,private,rec,sig,struct,then,to,true,try,type,val,virtual,when,while,with},
  keywords=[2]{Extrude, Perform, Plus, Int, Array, Genlet, FMA},
  sensitive=true,
  identifierstyle=\color{black},
  morecomment=[l]{--},
  morecomment=[l]{//},
  morecomment=[s]{(*}{*)},
  morestring=[b]",
  xleftmargin  = 2mm
}


\lstset{language=ocaml,style=style}

\newcommand{\function}[2]{\lambda{} #1. #2}
\newcommand{\continuation}[2]{\kappa{} #1. #2}

\newcommand{\Nat}[1]{\texttt{Nat}(#1)}
\newcommand{\Var}[2]{\texttt{Var}(#1_{#2})}
\newcommand{\Binder}[2]{#1_{#2}}

\newcommand{\Lam}[2]{\texttt{Lam}(#1, #2)}
\newcommand{\App}[2]{\texttt{App}(#1, #2)}
\newcommand{\Ret}[1]{\texttt{Ret}(#1)}
\newcommand{\Do}[3]{\texttt{Do}(#1, #2, #3)}
\newcommand{\Op}[1]{\texttt{Op}(#1)}
\newcommand{\Continue}[2]{\texttt{Continue}(#1, #2)}
\newcommand{\Hwith}[2]{\texttt{Hwith}(#1, #2)}
\newcommand{\Hret}[2]{\texttt{Hret}(#1, #2)}
\newcommand{\Hop}[4]{\texttt{Hop}(#1, #2, #3, #4)}
\newcommand{\err}[0]{\texttt{\textbf{err}}}

\newcommand{\return}[1]{\texttt{\textbf{return}} \,\, {#1}}
\newcommand{\op}[1]{\textbf{\texttt{op}}({#1})}
\newcommand{\bind}[3]{\texttt{\textbf{do}} \,\, {#1} \leftarrow {#2} \; \textbf{\texttt{in}} \; {#3}}
\newcommand{\handleWith}[2]{\textbf{\texttt{handle}} \,\, {#1} \,\, \textbf{\texttt{with}} \,\, \{{#2}\}}
\newcommand{\continue}[2]{\textbf{\texttt{continue}} \, {#1} \, {#2}}

\newcommand{\gensym}[1]{\textbf{\texttt{mkvar}} \, #1}
\newcommand{\varToAST}[1]{\return{{\texttt{Var}}({#1})}}

\newcommand{\dlet}[2]{\textbf{\texttt{dlet}}({#1}, {#2})}
\newcommand{\checkfv}[1]{\textbf{\texttt{check}}\, {#1}}
\newcommand{\checkm}[1]{\textbf{\texttt{check}}_{\textsf{M}}\, {#1}}
\newcommand{\tls}[1]{\textbf{\texttt{tls}}({#1})}

\newcommand{\freevars}[1]{{\textsf{FV}}^0({#1})}
\newcommand{\projfvs}[1]{\pi_{\texttt{Var}}({#1})}

\newcommand{\returnHandler}[2]{\textbf{\texttt{return}}(#1) \mapsto #2}
\newcommand{\opHandler}[3]{\textbf{\texttt{op}}(#1, #2) \mapsto #3}

\newcommand{\evalContext}[0]{E[-]}
\newcommand{\variableFrame}[2]{V_{#1}(#2)}

\newcommand{\equote}[1][e]{\langle \langle #1 \rangle \rangle}
\newcommand{\splice}[1][e]{\$ #1 }

\newcommand{\effconfiguration}[2]{\langle {#1} ; {#2} \rangle}
\newcommand{\transition}[2]{{#1} \leadsto {#2}}

\newenvironment{quoted}{\begin{mdframed}[linecolor=darkgrey]}{\end{mdframed}\par\vspace}

\makeatletter
\newcommand{\oset}[3][0ex]{%
  \mathrel{\mathop{#3}\limits^{
    \vbox to#1{\kern-2\ex@
    \hbox{$\scriptstyle#2$}\vss}}}}
\makeatother

\makeatletter
% issue another \@doendpe and lift it out of the group
\patchcmd{\mint@iii}
  {\minted@langlinenosoff\endgroup}
  {\minted@langlinenosoff\endgroup\@doendpe}
  {}{}
\makeatother

\makeatletter
\tcbset{
  after app={%
    \ifx\tcb@drawcolorbox\tcb@drawcolorbox@breakable
    \else
      % add only when not breakabel
      \@endparenv
    \fi
  }
}

% for breakable
\appto\tcb@use@after@lastbox{\@endparenv\@doendpe}
\makeatother

\DeclareRobustCommand\longtwoheadrightarrow
     {\relbar\joinrel\twoheadrightarrow}

\newcommand{\type}[3][]{\Gamma #1 \vdash #2 : #3}
\newcommand{\effectType}[2][\Delta]{{#2} \, ! \, {#1}}
\newcommand{\functionType}[3][\Delta]{{#2} \oset{\text{\tiny ${#1}$}}{\longrightarrow} {#3}}
\newcommand{\handlerType}[2]{#1 \Longrightarrow #2}
\newcommand{\continuationType}[3][\Delta]{#2 \oset{\text{\tiny ${#1}$}}{\longtwoheadrightarrow} #3}

% \newcommand\xrsquigarrow[1]{%
% \mathrel{%
% \begin{tikzpicture}[baseline= {( $ (current bounding box.south) + (0,-0.5ex) $ )}]
%   \node[inner sep=.5ex] (a) {$\scriptstyle #1$};
%   \path[draw,implies-,double distance between line centers=1.5pt,decorate,
%     decoration={zigzag,amplitude=0.7pt,segment length=1.2mm,pre=lineto,
%     pre   length=4pt}]
%     (a.south east) -- (a.south west);
% \end{tikzpicture}}%
% }

  % \newenvironment{codeblock}[2][][]{
%     \begin{tcblisting}[
%         minted language=ocaml,
%         minted options={mathescape, linenos, \#2},
%         \#1
%     ]
% }
% {\end{tcblisting}}

% \newenvironment{ocaml}{\begin{codeblock}}{\end{codeblock}}

% \newtcblisting{ocaml-box}{
%     listing only
% }

% \newenvironment{code}[1]
%  {\VerbatimEnvironment
%   \begin{minted}{#1}}
%  {\end{minted}}

% \newenvironment{ocaml}{%
%     \begin{code}{ocaml}
% }{
%     \end{code}
% }
% \newenvironment{macocaml}{\begin{code}{macocaml.py:MacocamlLexer}}{\end{code}}

% \renewcommand{\theFancyVerbLine}{\ttfamily \textcolor[rgb]{0.5,0.5,0.5}{\footnotesize{\arabic{FancyVerbLine}}}}

\DeclarePairedDelimiter\Brackets{\lBrack}{\rBrack}

\makeatletter
\tcbset{common/.style={
    enhanced,
    top=4pt,
    left=5pt,
    bottom=4pt,
    listing only,
    colframe=white,
  },
  after app={%
    \ifx\tcb@drawcolorbox\tcb@drawcolorbox@breakable
    \else
      % add only when not breakabel
      \@endparenv
    \fi
  }
  \appto\tcb@use@after@lastbox{\@endparenv\@doendpe}
}
\makeatother

\newtcblisting{ocaml}{
  common,
  colback=ocamlBackground,
  width=0.96\textwidth,
  before={\par\vspace{0.2\baselineskip}\noindent},
  after={\\
  \vspace{-4mm}},
  listing options = {language=ocaml, style=lst_style},
  overlay={\node[fill=ocamlHighlight,yshift=-7.8pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){OCaml};}
%   skin=tile,
 }

 \newtcblisting{ocamllst}{
  common,
  colback=ocamlBackground,
  width=0.96\textwidth,
  before={\par\vspace{0.2\baselineskip}\noindent},
  after={\par\vspace{0\baselineskip}\noindent},
  listing options = {language=ocaml,style=lst_style},
  overlay={\node[fill=ocamlHighlight,yshift=-7.8pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){OCaml};}
%   skin=tile,
 }

%  \newcommand{\macocamlLexer}{lexers/macocaml.py:MacocamlLexer}
 \newtcblisting{macocaml}{
  common,
  colback=ocamlBackground,
  width=0.96\textwidth,
  before={\par\vspace{0.2\baselineskip}\noindent},
  after={\\
  \vspace{-4mm}},
  listing options = {language=ocaml,style=lst_style},
  overlay={\node[fill=ocamlHighlight,yshift=-7.17pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){MacoCaml};}
%   skin=tile,
 }


 \newtcblisting{macocamllst}{
  common,
  colback=ocamlBackground,
  width=0.96\textwidth,
  before={\par\vspace{0\baselineskip}\noindent},
  after={\par\vspace{0\baselineskip}\noindent},
  listing options = {language=ocaml,style=lst_style},
  overlay={\node[fill=ocamlHighlight,yshift=-7.17pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){MacoCaml};}
%   skin=tile,
 }

 \newtcblisting{metaocaml}{
  common,
  colback=ocamlBackground,
  width=0.96\textwidth,
  after={\par\vspace{0.2\baselineskip}\noindent},
  listing options = {language=ocaml,style=lst_style},
  overlay={\node[fill=ocamlHighlight,yshift=-7.8pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){MetaOCaml};}
%   skin=tile,
 }
 \newtcblisting{metaocamllst}{
  common,
  colback=ocamlBackground,
  width=0.96\textwidth,
  % before={\par\vspace{0\baselineskip}\noindent},
  after={\par\vspace{0\baselineskip}\noindent},
  listing options = {language=ocaml,style=lst_style},
  overlay={\node[fill=ocamlHighlight,yshift=-7.8pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){MetaOCaml};}
%   skin=tile,
 }

  \newtcblisting{stdout}{
  listing only,
  colframe=white,
  % minted language=ocaml,
  colback=white,
  fontupper=\linespread{1.1}\normalsize,
  before={\par\vspace{0\baselineskip}\noindent},
  after={\par\vspace{0\baselineskip}\noindent},
  listing options = {style=plain,language=plain}
  % listing engine=minted,
  % minted options = {linenos, fontsize=\footnotesize, numbersep=15pt, baselinestretch=1.1, escapeinside=!!},
  % overlay={\node[fill=effHighlight,yshift=-8.8pt,xshift=-10pt,left,text=white,
  %        anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){$\mathbf{\lambda}_{\text{op}}$};}
%   skin=tile,
 }




 \newcommand{\efflang}{$\lambda_{\texttt{op}}$}
 \newcommand{\sourceLang}{$\lambda_{\equote[\texttt{op}]}$}
 \newcommand{\calculusName}{\sourceLang}
 \newcommand{\coreLang}{$\lambda_{\texttt{AST}(\texttt{op})}$}
 \newcommand{\recLang}{\sourceLang$^{\gamma}$}


 \newtcolorbox{eff-i}{
  common,
  % minted language=ocaml,
  colback=effBackground,
  width=0.96\textwidth,
  fontupper=\linespread{1.1}\listingfontsize,
  after={\par\vspace{0.2\baselineskip}\noindent},
  % listing engine=minted,
  % minted options = {linenos, fontsize=\footnotesize, numbersep=15pt, baselinestretch=1.1, escapeinside=!!},
  overlay={\node[fill=effHighlight,yshift=-8.6pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){$\mathbf{\lambda}_{\text{op}}$};}
%   skin=tile,
 }

 \newtcolorbox{efflst-i}{
  common,
  % minted language=ocaml,
  colback=effBackground,
  width=0.96\textwidth,
  fontupper=\linespread{1.1}\listingfontsize,
  after={\par\vspace{0\baselineskip}\noindent},
  % listing engine=minted,
  % minted options = {linenos, fontsize=\footnotesize, numbersep=15pt, baselinestretch=1.1, escapeinside=!!},
  overlay={\node[fill=effHighlight,yshift=-8.6pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){$\mathbf{\lambda}_{\text{op}}$};}
%   skin=tile,
 }

 \newtcolorbox{eff-desc-i}{
  common,
  % minted language=lexers/macocaml.py:MacocamlLexer,
  colback=white,
  fontupper=\small,
  borderline north={0.5mm}{0mm}{effHighlight,line width=1pt},
borderline south={0.5mm}{0mm}{effHighlight,line width=1pt},
  overlay={\node[fill=effHighlight,yshift=-8pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){$\mathbf{\lambda}_{\text{op}}$};}
%   skin=tile,
 }

    \newenvironment{eff}{
  \begin{eff-i}
 }{  \end{eff-i}}

   \newenvironment{efflst}{
  \begin{efflst-i}
 }{  \end{efflst-i} \\
 \vspace{-3mm}}

 \newenvironment{eff-desc}{
  \begin{eff-desc-i}
 }{  \end{eff-desc-i} \vspace{-4mm}}

 \newtcolorbox{source-i}{
  common,
  % minted language=ocaml,
  colback=sourceBackground,
  width=0.96\textwidth,
  fontupper=\linespread{1.1}\listingfontsize,
  after={\par\vspace{0.2\baselineskip}\noindent},
  % listing engine=minted,
  % minted options = {linenos, fontsize=\footnotesize, numbersep=15pt, baselinestretch=1.1, escapeinside=!!},
  overlay={\node[fill=sourceHighlight,yshift=-8.7pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){\sourceLang{}};}
%   skin=tile,
 }

  \newtcolorbox{sourcelst-i}{
  common,
  % minted language=ocaml,
  colback=sourceBackground,
  width=0.96\textwidth,
  fontupper=\linespread{1.1}\listingfontsize,
  after={\par\vspace{0\baselineskip}\noindent},
  % listing engine=minted,
  % minted options = {linenos, fontsize=\footnotesize, numbersep=15pt, baselinestretch=1.1, escapeinside=!!},
  overlay={\node[fill=sourceHighlight,yshift=-8.7pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){\sourceLang{}};}
%   skin=tile,
 }


 \newtcolorbox{source-desc-i}{
  common,
  % minted language=lexers/macocaml.py:MacocamlLexer,
  colback=white,
  fontupper=\small,
  borderline north={0.5mm}{0mm}{sourceHighlight,line width=1pt},
borderline south={0.5mm}{0mm}{sourceHighlight,line width=1pt},
  overlay={\node[fill=sourceHighlight,yshift=-8.1pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){\sourceLang{}};}
%   skin=tile,
 }

 \newenvironment{source}{
  \begin{source-i}
 }{  \end{source-i}\\
      \vspace{-4mm}}

   \newenvironment{sourcelst}{
  \begin{sourcelst-i}
 }{  \end{sourcelst-i}\\
      \vspace{-4mm}}

  \newenvironment{source-desc}{
  \begin{source-desc-i}
 }{  \end{source-desc-i} \vspace{-4mm}}

 \newtcolorbox{core-i}{
  common,
  % minted language=ocaml,
  colback=coreBackground,
  width=0.96\textwidth,
  fontupper=\linespread{1.1}\listingfontsize,
  after={\par\vspace{0.2\baselineskip}\noindent},
  % listing engine=minted,
  % minted options = {linenos, fontsize=\footnotesize, numbersep=15pt, baselinestretch=1.1, escapeinside=!!},
  overlay={\node[fill=coreHighlight,yshift=-8.7pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){\coreLang{}};}
%   skin=tile,
 }

  \newtcolorbox{corelst-i}{
  common,
  % minted language=ocaml,
  colback=coreBackground,
  width=0.96\textwidth,
  fontupper=\linespread{1.1}\listingfontsize,
  after={\par\vspace{0\baselineskip}\noindent},
  % listing engine=minted,
  % minted options = {linenos, fontsize=\footnotesize, numbersep=15pt, baselinestretch=1.1, escapeinside=!!},
  overlay={\node[fill=coreHighlight,yshift=-8.7pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){\coreLang{}};}
%   skin=tile,
 }

  \newtcolorbox{core-desc-i}{
  common,
  % minted language=lexers/macocaml.py:MacocamlLexer,
  colback=white,
  fontupper=\small,
  borderline north={0.5mm}{0mm}{coreHighlight,line width=1pt},
borderline south={0.5mm}{0mm}{coreHighlight,line width=1pt},
  overlay={\node[fill=coreHighlight,yshift=-8.1pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){\coreLang{}};}
%   skin=tile,
 }

  \newenvironment{core}{
  \begin{core-i}
 }{  \end{core-i}\\ \vspace{-4mm}}

   \newenvironment{corelst}{
  \begin{corelst-i}
 }{  \end{corelst-i}\\ \vspace{-4mm}}

   \newenvironment{core-desc}{
  \begin{core-desc-i}
 }{  \end{core-desc-i} \vspace{-4mm}}

 \newtcolorbox{rec-i}{
  common,
  % minted language=ocaml,
  colback=recBackground,
  width=0.96\textwidth,
  fontupper=\linespread{1.1}\listingfontsize,
  after={\par\vspace{0.2\baselineskip}\noindent},
  % listing engine=minted,
  % minted options = {linenos, fontsize=\footnotesize, numbersep=15pt, baselinestretch=1.1, escapeinside=!!},
  overlay={\node[fill=recHighlight,yshift=-8.9pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){\recLang{}};}
%   skin=tile,
 }

  \newtcolorbox{reclst-i}{
  common,
  % minted language=ocaml,
  colback=recBackground,
  width=0.96\textwidth,
  fontupper=\linespread{1.1}\listingfontsize,
  after={\par\vspace{0\baselineskip}\noindent},
  % listing engine=minted,
  % minted options = {linenos, fontsize=\footnotesize, numbersep=15pt, baselinestretch=1.1, escapeinside=!!},
  overlay={\node[fill=recHighlight,yshift=-8.9pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){\recLang{}};}
%   skin=tile,
 }

\newtcolorbox{rec-desc-i}{
  common,
  % minted language=lexers/macocaml.py:MacocamlLexer,
  colback=white,
  fontupper=\small,
  borderline north={0.5mm}{0mm}{recHighlight,line width=1pt},
borderline south={0.5mm}{0mm}{recHighlight,line width=1pt},
  overlay={\node[fill=recHighlight,yshift=-8.1pt,xshift=-10pt,left,text=white,
         anchor=east,font=\scriptsize\ttfamily\bfseries] at (frame.north east){\recLang{}};}
%   skin=tile,
 }

   \newenvironment{rec}{
  \begin{rec-i}
 }{  \end{rec-i}\\ \vspace{-4mm}}

   \newenvironment{reclst}{
  \begin{reclst-i}
 }{  \end{reclst-i}\\ \vspace{-4mm}}

 \newenvironment{rec-desc}{
  \begin{rec-desc-i}
 }{  \end{rec-desc-i} \vspace{-4mm}}

 \newenvironment{code}{\centering}{\par\vspace{0.6\baselineskip}}

 \makeatletter
\newcommand\colorwave[1][blue]{\bgroup \markoverwith{\lower3.5\p@\hbox{\sixly \textcolor{#1}{\char58}}}\ULon}
\font\sixly=lasy6 % does not re-load if already loaded, so no memory problem.
\makeatother

\DeclareFloatingEnvironment[name = {Typing Derivation}]{typederivation}
\Crefname{typederivation}{Typing Derivation}{Typing Derivations}
\crefname{typederivation}{typing derivation}{typing derivations}

\DeclareFloatingEnvironment[name = {Listing}]{floatinglisting}

\newcommand{\hl}[1]{\colorbox{yellow}{#1}}
\newcommand{\fadedHL}[1]{\colorbox{fadedYellow}{#1}}


\newcommand{\rulename}[2]{(\textsc{{#1}-{#2}})}
\newcommand{\reductionRule}[1]{\rulename{Red}{#1}}
\newcommand{\congruenceRule}[1]{\rulename{Cng}{#1}}
\newcommand{\effectRule}[1]{\rulename{Eff}{#1}}

\newcommand{\novelCheck}{C4C}
\newcommand{\NovelCheck}{C4C}

\renewenvironment{leftbar}[2][\hsize]
{
    \def\FrameCommand
    {
        {\color{#2}\vrule width 3pt}
        \hspace{4pt}
    }
    \MakeFramed{\hsize#1\advance\hsize-\width\FrameRestore}
}
{\endMakeFramed}

\ifdefined\EXTENDED
\newcommand{\unextendedOnly}[1]{}
\newcommand{\extendedOnly}[1]{#1}
\newenvironment{extendedonly}{}{}
\else
\newcommand{\unextendedOnly}[1]{#1}
\newcommand{\extendedOnly}[1]{}
\newenvironment{extendedonly}{\expandafter\comment}{\expandafter\endcomment}
\fi


==> sty/scope-pkg.tex <==
\usepackage{url}
\usepackage{hyperref}
\usepackage{latexsym}
% \usepackage{catchfile}
\usepackage[export]{adjustbox}
\usepackage{newfloat}

% MATH
\usepackage{amsmath, amsfonts, mathtools}
% \usepackage[amsmath,thmmarks,framed]{ntheorem} 
\usepackage{framed}
\usepackage{mathpartir}
\usepackage{centernot}

% DISPLAY
\usepackage{xcolor}
\usepackage[inline]{enumitem}
%% \usepackage{titlesec}
\usepackage{xspace}

\setcounter{secnumdepth}{3}

\newcounter{listing}
\DeclareFloatingEnvironment[
    name=Listing
]{listing}

% FONTS
% \usepackage{anyfontsize}
\usepackage[normalem]{ulem}
% \usepackage{bold-extra}
% \usepackage{inconsolata}

% CITATIONS
\usepackage{natbib}
\usepackage{booktabs}

% FIGURES
\usepackage{subcaption}
\usepackage{wrapfig}

% TABLES
\usepackage{multirow}
\usepackage{tabularx}
\usepackage{hhline}

% CODE
\usepackage{listings}
\usepackage{algorithm}
\usepackage{algpseudocode}

% VISUALS
\usepackage{tcolorbox}
\tcbuselibrary{hooks, listings, breakable, skins}

\usepackage{etoolbox}

% \usepackage{tikz-qtree}
% \usepackage{tikz-qtree-compat}
\usepackage[hypcap=false]{caption}

% \usepackage{array}
% \usepackage{colortbl}
% \tcbuselibrary{skins}


% 
% 


% \usepackage{breakurl}

% \usepackage{graphicx}
% \usepackage{subcaption}
% \usepackage{caption}
% \usepackage{svg}

% \usepackage{booktabs}
% \usepackage{longtable}

% \usepackage[separate-uncertainty, binary-units]{siunitx}



\usepackage{tikz}
\usetikzlibrary{automata, positioning, arrows, trees, calc,decorations.pathmorphing,decorations.pathreplacing,shapes}
\usetikzlibrary{backgrounds}

\tikzset{snake it/.style={decorate, decoration=snake}}

\usepackage{import}

% CROSS-REFERENCES
\usepackage[nameinlink]{cleveref}

% \mdfsetup{%
% topline=false,
% rightline=false,
% bottomline=false,
% linewidth=3pt,
% innerleftmargin=15pt,
% innerrightmargin=0pt,
% skipabove=\baselineskip,
% skipabove=1.2\baselineskip,
% }

% \newtheoremstyle{break}
%   {\topsep}{\topsep}%
%   {\itshape}{}%
%   {\bfseries}{}%
%   {\newline}{}%
% \theoremstyle{break}

% \newtheorem{theorem}{Theorem}

\newtheorem{mdtheorem}{Theorem}[section]
% \newenvironment{theorem}[2][]%
%    {\vspace{0\baselineskip}\begin{theorem}[#1]}
%    {\end{theorem}\par\vspace{\baselineskip}}

\newtheorem{mdcorollary}[mdtheorem]{Corollary}
\newenvironment{corollary}[1][]%
  {\begin{mdcorollary}[#1]}
  {\end{mdcorollary}}

\newtheorem{mddefinition}[mdtheorem]{Definition}
\newenvironment{definition}[1][]%
    {\begin{mddefinition}[#1]}
    {\end{mddefinition}}

    \newtheorem{mdinduction}[mdtheorem]{Induction Principle}
\newenvironment{inductionPrinciple}[1][]%
    {\begin{mdinduction}[#1]}
    {\end{mdinduction}}

    \newtheorem{mdlemma}[mdtheorem]{Lemma}
\newenvironment{lemma}[1][]%
    {\begin{mdlemma}[#1] 
    }
    {\end{mdlemma}}

% % \usepackage{pgfplots, pgfplotstable}

% \usepackage{minted}

% \usepackage[framemethod=TikZ]{mdframed}
% \usepackage{textcomp}
% \usepackage{enumitem}



% \usepackage{alltt}

% \usepackage{listings}

% \usepackage{etoolbox}

% \usepackage{scrhack}

% \usepackage{algpseudocode}

% \usepackage{bussproofs}

% \usepackage{multirow}
% \usepackage{multicol}

% \usepackage{fancyhdr}

\crefformat{section}{#2\S#1#3}
\Crefformat{section}{#2\S#1#3}
